Semiparametric curve alignment and shift density estimation for biological data

Assume that we observe a large number of curves, all of them with identical, although unknown, shape, but with a different random shift. The objective is to estimate the individual time shifts and their distribution. Such an objective appears in several biological applications like neuroscience or ECG signal processing, in which the estimation of the distribution of the elapsed time between repetitive pulses with a possibly low signal-noise ratio, and without a knowledge of the pulse shape is of interest. We suggest an M-estimator leading to a three-stage algorithm: we split our data set in blocks, on which the estimation of the shifts is done by minimizing a cost criterion based on a functional of the periodogram; the estimated shifts are then plugged into a standard density estimator. We show that under mild regularity assumptions the density estimate converges weakly to the true shift distribution. The theory is applied both to simulations and to alignment of real ECG signals. The estimator of the shift distribution performs well, even in the case of low signal-to-noise ratio, and is shown to outperform the standard methods for curve alignment.

==> Notations.tex <==
%
%
% Fichier avec les notations et les definitions d'environnement
%
%

\newcommand{\funcnorm}[2]{\left\| #1 \right\|_{#2}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations MathÈmatiques %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\rme{\mathrm{e}}    % Fonction exponentielle
\def\rmi{\mathrm{i}}    % Imaginaire Pur
\def\nset{\mathbb{N}} % Entiers naturels
\def\zset{\mathbb{Z}} % Entiers relatifs
\def\rset{\mathbb{R}} % RÈels
\def\qset{\mathbb{Q}} % Rationnels
\def\cset{\mathbb{C}} % Complexes
\def\PP{\mathbb{P}}             % Espaces de proba
\def\E{\mathbb{E}}              % EspÈrance d'une var
\def\Var{\mathrm{Var}}  

%\usepackage{ifthen}
%\newboolean{pdf}        % Are we using pdftex?
%\ifx\pdfoutput\undefined
%  \setboolean{pdf}{false}       % Not running pdflatex
%  \def\1{\mathbbm{1}}
%\else
%  \setboolean{pdf}{true}        % Running pdflatex
%  \pdfoutput=1
%  \def\1{\mathbf{1}}          % mathbbm semble pas marcher avec pdflatex
%  \def\1{\mathbbm{1}}
%\fi

\newcommand{\eqsp}{\;}

\newcommand{\eqdef}{\ensuremath{\stackrel{\mathrm{\Delta}}{=}}}

%%%%%%%%%%%%%%%%%%
% Fonctionnelles %
%%%%%%%%%%%%%%%%%%

\newcommand{\funk}[2]{\rho(#1,#2)}
\newcommand{\funkname}{\rho}
\newcommand{\funkd}{F_p}
\newcommand{\dcdf}[2]{k(#1,#2)}
\newcommand{\dcdfname}{k}
\newcommand{\dcdfconv}[3]{k^{\stackrel{(2)}{*} #3} (#1,#2)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations pour la these %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\densexp}[1]{{\cal E}_{#1}}
\newcommand{\cumenergie}[1]{\bar{E}_{#1}}
\newcommand{\workload}[1]{S_{#1}}
\newcommand{\sampleperiod}{T_e}
\newcommand{\discretesignal}[1]{s(#1)}
\newcommand{\period}[1]{T_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TransformÈes de Laplace %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\laptot}{{\cal L}}
\newcommand{\lapone}{{\cal L}_U}
\newcommand{\laptwo}{{\cal L}_E}

% Version discrete
\newcommand{\TZ}[1]{\mathcal{TZ}(#1)} 

% Version Fourier
\newcommand{\TF}[1]{#1^*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Variables d'intÈgration et variables muettes %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\realone}{x}
\newcommand{\realtwo}{y}
\newcommand{\compone}{s}
\newcommand{\comptwo}{p}
\newcommand{\intone}{m}
\newcommand{\inttwo}{n}

\newcommand{\intonemute}{i}
\newcommand{\inttwomute}{j}

\newcommand{\realonemute}{\tau}
\newcommand{\realonemutebis}{u}
\newcommand{\realtwomute}{\varepsilon}
\newcommand{\componemute}{\omega}
\newcommand{\comptwomute}{\nu}
\newcommand{\convergeabs}{c}


%%%%%%%%%%%%%%%%%%%%%%%%%%
% Noyaux de l'estimateur %
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\kernel}{K}
\newcommand{\TFkernel}{K^*}
\newcommand{\bandwidth}{h}
\newcommand{\timelimit}{T}

%%%%%%%%%%%%%%%%%%%%%%
% Pour la loi ideale %
%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\poissid}{\mathcal{N}}

\newcommand{\densid}{f}
\newcommand{\measid}{P}

\newcommand{\funcid}{f_{(U,E)}}

\newcommand{\sampleid}{\{(X_k,Y_k)\}}

\newcommand{\temps}[1]{T_{#1}}
\newcommand{\genericduree}{X}
\newcommand{\genericenergie}{Y}
\newcommand{\duree}[1]{X_{#1}}
\newcommand{\energie}[1]{Y_{#1}}
\newcommand{\couple}[1]{(X_{#1},Y_{#1})}
\newcommand{\marginald}{\pi}
\newcommand{\marginal}{m}
\newcommand{\TFmarginal}{m^*}

% Version discrete
\newcommand{\tempsd}[1]{T_{#1}^{~(d)}}
\newcommand{\dureed}[1]{X_{#1}^{~(d)}}
\newcommand{\energied}[1]{Y_{#1}^{~(d)}}
\newcommand{\coupled}[1]{(X_{#1}^{~(d)},Y_{#1}^{~(d)})}

%%%%%%%%%%%%%%%%%%%%%%%
% Pour la loi observee %
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\poissobs}{(N_t')_{t\geq 0}}

\newcommand{\densobs}{g}
\newcommand{\measobs}{P'}

\newcommand{\funcobs}{f_{(u,e)}}
\newcommand{\sampleobs}{\{(X'_k, Y'_k)\}}
\newcommand{\genericdureeo}{X'}
\newcommand{\genericenergieo}{Y'}
\newcommand{\tempso}[1]{T'_{#1}}
\newcommand{\dureeo}[1]{X'_{#1}}
\newcommand{\energieo}[1]{Y'_{#1}}
\newcommand{\coupleo}[1]{(X'_{#1},Y'_{#1})}
% Pour les mesures de proba associees aux densites...
\newcommand{\probmeas}[1]{\mathrm{P} #1}
\newcommand{\empmeas}{\hat{P}_{n}}
% Pour la version discrete
\newcommand{\tempsod}[1]{T_{#1}^{\prime~(d)}}
\newcommand{\dureeod}[1]{X_{#1}^{\prime~(d)}}
\newcommand{\energieod}[1]{Y_{#1}^{\prime~(d)}}


%%%%%%%%%%%%%%%%%%
% Pour les idles %
%%%%%%%%%%%%%%%%%%

\newcommand{\genericidle}{Z}
\newcommand{\idle}[1]{Z_{#1}}
\newcommand{\idled}[1]{Z_{#1}^{\prime~(d)}}


%%%%%%%%%%%%%%%%%%%%%%%%%
% Dummy variables
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\auxvar}{\tilde{\lambda}}
\newcommand{\densvar}{\tilde{\densobs}}
\newcommand{\measvar}{\tilde{P}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition des graphiques PostScript %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rayonphotonique}{%
\begin{pspicture}(7.5,2)
\psline[linearc=0.25]{*->}%
(0,1)(0.5,0.5)(1,1)(1.5,1.5)(2,1)(2.5,0.5)(3,1)(3.5,1.5)(4,1)(4.5,0.5)(5,1)(5.5,1.5)(6,1)(6.5,0.5)(7,1)(7.5,1)
\end{pspicture}}

\newcommand{\fleche}{%
\begin{pspicture}(7.5,2)
\psline{->}%
(0,1)(7.5,1)
\end{pspicture}}

